DeepMesh: Differentiable Iso-Surface Extraction

Geometric Deep Learning has recently made striking progress with the advent of continuous deep implicit fields. They allow for detailed modeling of watertight surfaces of arbitrary topology while not relying on a 3D Euclidean grid, resulting in a learnable parameterization that is unlimited in resolution. Unfortunately, these methods are often unsuitable for applications that require an explicit mesh-based surface representation because converting an implicit field to such a representation relies on the Marching Cubes algorithm, which cannot be differentiated with respect to the underlying implicit field. In this work, we remove this limitation and introduce a differentiable way to produce explicit surface mesh representations from Deep Implicit Fields. Our key insight is that by reasoning on how implicit field perturbations impact local surface geometry, one can ultimately differentiate the 3D location of surface samples with respect to the underlying deep implicit field. We exploit this to define DeepMesh - an end-to-end differentiable mesh representation that can vary its topology. We validate our theoretical insight through several applications: Single view 3D Reconstruction via Differentiable Rendering, Physically-Driven Shape Optimization, Full Scene 3D Reconstruction from Scans and End-to-End Training. In all cases our end-to-end differentiable parameterization gives us an edge over state-of-the-art algorithms.

==> fig/cfd_mult_opt.tex <==
\begin{figure}[t]
		\vspace{-5pt}
		\begin{center}
		%,grid,tics=5
			\begin{overpic}[clip, trim=4.0cm 3.0cm 2.0cm 3.0cm, width= 0.7\textwidth]{figures/cfd_mult_opts.png}
    			\put(45,35){\small{Cabin at the back}}
    			\put(45,18,5){\small{Cabin at the front}}
    			\put(45,2){\small{No constraints}}
			\end{overpic}
		\end{center}
		\vspace{-5pt}
		\caption{\textbf{Drag optimization with different constraints.}
	     The figure shows the results of optimizations with the same initial shape (left image) but different mesh-constraints. The rows of images contain renderings of the surfaces obtained on different optimization steps. The top row corresponds to an optimization run with a constraint for surface to contain a sphere of a certain radius at the back half - represents a driver space. For the middle row the same sphere was put in the front half of the car. Finally in the third-row experiment we did not introduce any constraints. \PB{We say at some point that without constraints, the optimization would collapse to 0. I understand that here we have this regularization procedure etc..., but still, it will raise questions. Can we just remove the not constrained one?}\ER{I am working on visualizing constraints, as I don't find "Cabin at the back", "cabin at the front" very informative", but see comment below}
	    }
\label{fig:cfd_mult_opt}
\end{figure}

==> fig/fig_dim.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{wrapfigure}[12]{l}{50mm}
			\begin{overpic}[clip, trim=8.0cm 7cm 17cm 6.5cm,width=0.3\textwidth]{fig/fig_dim.pdf}
			\put(8,4){\small{$\{s = 0\} $}}
			\put(0,23){\small{$\{s +  \Delta s = 0\} $}}
			\put(67,23){$\mathbf p$}
			\put(64,39){$\mathbf n (\mathbf p)$}
			\put(41,52){$\mathbf p'$}
			\put(26,64){$\mathbf n (\mathbf p')$}
			\end{overpic}
		\caption{Geometric relation between local surface change $\Delta \mathbf p = \mathbf p' - \mathbf p$ and signed distance field perturbation  $\Delta s$.	\vspace{2.0cm}}
		\vspace{2.0cm}
		\label{fig:dim}
\end{wrapfigure}

==> fig/fig_implementation.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
            \begin{center}
            %,grid,tics=5
			\begin{overpic}[clip, trim=0.0cm 0cm 0cm 0cm,width=0.4\textwidth]{fig/fig_implementation_p.pdf}
			\end{overpic} 
			\end{center}
	\vspace{-6mm}
	\caption{\textbf{Accelerating isosurface extraction.} The blue curve depicts the run-time or our naive implementation as a function of grid resolution while the red curve depicts that of the accelerated version.}
	\label{fig:implementation}
\end{figure}

==> fig/fig_pix3D.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
        % \vspace{-4pt}
		\begin{center}
		% ,grid,tics=5
			\begin{overpic}[clip, trim=13.0cm 10cm 6cm 0.5cm,width=0.5\textwidth]{fig/fig_Pix3D_p.pdf}
			\put(5,2){\small{Input }}
			\put(33,2){\small{DISN} \cite{Xu19b}}
			\put(67,2){\small{\textit{DeepMesh} (Ours) }}

			\end{overpic}
		\end{center}
		\vspace{-14pt}
		\caption{\textbf{Pix3D Reconstructions.} We compare our refined predictions to the runner-up approach for the experiment in Tab. \ref{tab:pix3d}. \textit{DeepMesh} can represent arbitrary topology as well as learn strong shape priors, resulting in reconstructions that are consistent even when observed from view-points different from the input one. {For more results, and a visual demonstration of the impact of refinement on 3D reconstructions, see Appendix.}%\bg{Here we show results of our method using an SDF as underlying field, and refine 2D contours locations.} 
		}
\label{fig:pix3D}
\vspace{-3pt}
\end{figure}

==> fig/fig_proof.tex <==
\begin{figure*}[t]
\vspace{-6pt}
            \begin{center}
            %,grid,tics=5
			\begin{overpic}[clip, trim=2.0cm 10cm 10cm 2cm,width=0.7\textwidth]{fig/fig_proof_pdf.pdf}
		
			\put(-10,1){\small{$\{s = 0\} $}}
			\put(-20,10){\small{$\{s +  \Delta s = 0\} $}}
			\put(14.5,8){$\mathbf v$}
			\put(14,14){$\mathbf n (\mathbf v)$}
			\put(5,19){$\mathbf v'$}
			\put(-1,24){$\mathbf n (\mathbf v')$}
			
			\put(48,8){$\mathbf v$}
			\put(48,12){$\mathbf n (\mathbf v)$}
			\put(45,16){$\mathbf v'$}
			\put(40,21){$\mathbf n (\mathbf v')$}
			
			\put(83,8){$\mathbf v$}
			\put(77,15){$\mathbf n (\mathbf v) = - \frac{\partial \mathbf v}{\partial s} $}
			
			\put(45,31){$\Delta s \rightarrow 0$}
			
			
			
			\end{overpic} 
			\end{center}
	\vspace{-3mm}
	\caption{\textbf{Iso-surface differentiation.} We adopt a \textit{continuous} model in terms of how small perturbations of a signed distance function locally impact surface geometry. Here, we depict the geometric relation between local surface change $\Delta \mathbf v = \mathbf v' - \mathbf v$ and a signed distance perturbation  $\Delta s < 0$, which we exploit to compute $\frac{\partial \mathbf v}{\partial s}$ in the formal derivation below.}
		\label{fig:mc_proof}
\end{figure*}

==> fig/fig_svr.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
        \vspace{-8pt}
		\begin{center}
		%
			\begin{overpic}[clip, trim=0.0cm 14cm 0 0.5cm,width=1.0\textwidth]{fig/fig_svr_p.pdf}
			\put(6,14.5){\small{Input }}
			\put(15,14.5){\small{\textit{MeshSDF} Raw}}
			\put(35,14.5){\small{refinment iterations}}
			\put(60.5,15.5){\small{target}}
			\put(59,13.5){\small{silhouette}}
			\put(74,14.5){\small{\textit{MeshSDF} Refined}}
			\end{overpic}
		\end{center}
		\vspace{-8pt}
		\caption{\textbf{Shilouette-driven refinment.} (a) given an input image, we exploit the differentiability of \textit{MeshSDF} to refine the predicted surface so that to match target silhouette in image space through Differentiable Rasterization \cite{Kato18}. }
\label{fig:svr}
\vspace{-6pt}
\end{figure}

==> fig/optimization_full.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
		\vspace{0pt}
		\begin{center}
		%,grid,tics=5
			\begin{overpic}[clip, trim=2.5cm 7.0cm 2.0cm 0.0cm, width=\textwidth]{fig/optimization_full_p.png}
    			\put(50,6){\small{optimization}}
    			\put(50,19){\small{optimization}}
    			\put(50,32){\small{optimization}}
    			
    			\put(96, 36){\small{$p_{max}$}}
    			\put(96, 27){\small{$0$}}
    			\put(96, 19.5){\small{$p_{min}$}}
    			
    			\put(-3, 34){\small{(a)}}
    			\put(-3, 23){\small{(b)}}
    			\put(-3, 8){\small{(c)}}
    			
    			
    			\put(72, 43.5){\small{optimized shape}}
    			\put(18, 43.5){\small{initial shape}}
    			
    			\put(11, 41){\small{simulated $p$}}
    			\put(26, 41){\small{predicted $p$}}
    			\put(75, 41){\small{predicted $p$}}
			\end{overpic}
		\end{center}
		\vspace{-4mm}
\caption{\textbf{Drag minimization.} We start with three random ShapeNet cars and minimize our objective function $\mathcal{L}_{task}$ with respect to the latent vector $\bz$ that describes them. In the first column, we show the initial shape as seen from the side, front, and top with the colors representing the pressure field $p$ predicted by the network $g_\beta$. The intermediate columns depict intermediate stages of the minimization. The last column depicts the final result. Note that the car at the bottom initially has a spoiler, which the optimizer removes. In other words, it turns a surface of genus-1 into one of genus-0. This is reverse of what we did in Fig.~\ref{fig:sanity} and would have been just as hard to do with earlier techniques that require an explicit mesh representation.} 
\label{fig:cfd_optimization_full}
\end{figure}

\comment{

	
	     We visualize our full constrained drag minimization pipeline for different initial shapes.
	     On the left-most column, we illustrate the ground-truth pressure field on the initial shape as computed by OpenFoam. On its right, the one predicted by our differentiable emulator. In the middle we visualize optimization iterations. Finally, on the right-most column, we depict the optimized car shape together with the pressure field predicted by the emulator.
	     Observe that, for the minimization in (c), we start with a shape with a spoiler (genus-1) and end up with a more aerodynamic car with different topology (genus-0).
	     This change of topology could not have been possible using \textit{classical} explicit surface parameterizations \cite{Baque18, Umetani18}. \ER{Switching to Figure with comparison to  \cite{Baque18, Umetani18}!!!}
	     
	     }

==> tables/end2end.tex <==

\begin{table}[ht]
	% 	\newcolumntype{Z}{S[table-format=1.3,table-auto-round]}
		\centering
		\small
		\caption{\textbf{End-to-end training.} We exploit end-to-end-differentiability to fine-tune pre-trained \textit{DeepSDF} networks so that to that to minimize directly our metric of interest, Chamfer distance ($\cdot 10^4$).}
		\label{table:end2end}
		%@{\hspace{6mm}}@{\hspace{2mm}}
		\begin{tabularx}{\linewidth}{@{}X*1{@{\hspace{2mm}}c}@{\hspace{3mm}}c@{\hspace{2mm}}c@{}}%{c|cc}
			\toprule
			Category &  DeepSDF &  DeepMesh \\
			\midrule
			Cars (train)  &  7.1 & \textbf{6.4} ($\downarrow 9 \%$)  \\
			Chairs (train) &  14.5 & \textbf{13.3} ($\downarrow 8 \%$) \\
			\midrule
			Cars (test)  &  8.4  & \textbf{6.7} ($\downarrow 20 \%$)\\
			Chairs (test) &  40.7  & \textbf{25.9} ($\downarrow 36 \%$) \\
			\bottomrule
		\end{tabularx}
	\end{table}
